Sparse Coding Frontend for Robust Neural Networks

Deep Neural Networks are known to be vulnerable to small, adversarially crafted, perturbations. The current most effective defense methods against these adversarial attacks are variants of adversarial training. In this paper, we introduce a radically different defense trained only on clean images: a sparse coding based frontend which significantly attenuates adversarial attacks before they reach the classifier. We evaluate our defense on CIFAR-10 dataset under a wide range of attack types (including Linf , L2, and L1 bounded attacks), demonstrating its promise as a general-purpose approach for defense.

==> arxiv/abstract.tex <==
%!TEX root = ms.tex

Deep Neural Networks are known to be vulnerable to small, adversarially crafted, perturbations. The current most effective defense methods against these adversarial attacks are variants of adversarial training. 
In this paper, we introduce a radically different defense trained only on clean images: a sparse coding based frontend which significantly attenuates adversarial attacks before they reach the classifier.
We evaluate our defense on CIFAR-10 dataset under a wide range of attack types (including $\ell^{\infty}$, $\ell^2$, and $\ell^1$ bounded attacks),
demonstrating its promise as a general-purpose approach for defense.


==> arxiv/ack.tex <==
%!TEX root = ms.tex


\subsection*{Acknowledgment}

This work was supported in part by the Army Research Office under grant W911NF-19-1-0053, and by the National Science Foundation under grants CIF-1909320 and CNS-1518812.



==> arxiv/background.tex <==
%!TEX root = ms.tex

\section{Adversarial Attacks}

{\bf Whitebox attacks} assume that the adversary has access to the model and its weights. For typical $\ell^p$ bounded attack models, 
projected gradient descent (PGD) is currently known to be the strongest. The $\ell^p$ budget $\epsilon$ is divided into smaller steps $\delta$. In each step, gradient of the loss function $\mathcal{L}$ with respect to the input is normalized and scaled by $\delta$, and added to the perturbation calculated in the previous step. After each step, the computed attack is clipped to conform to the $\ell^p$ bound. Mathematically, PGD can be written as
\vspace*{-0.2cm}
\begin{equation}\label{eq:PGD}
\mathbf{e}_{i+1} = \text{clip}^p_{\epsilon}\big[\mathbf{e}_{i}+\delta \cdot \frac{\nabla_\mathbf{e} \mathcal{L}(\mathbf{f}(\mathbf{x}+\mathbf{e}_i),\mathbf{y})}{||(\nabla_\mathbf{e} \mathcal{L}(\mathbf{f}(\mathbf{x}+\mathbf{e}_i),\mathbf{y})||_p}\big]
\end{equation}
where $\mathbf{x}$ is the input, $\mathbf{y}$ is the target output, and $\mathbf{e}_i$ is the adversarial perturbation calculated in step $i$. The loss function $\mathcal{L}$ is usually taken as the cross-entropy loss between the network outputs $\mathbf{f}(\mathbf{x})$ and target output $\mathbf{y}$. Through \eqref{eq:PGD}, gradient ascent over the loss in the input space is achieved.

To optimize over a greater area in the input space, the attack can be initialized with random restarts within the $\epsilon$ $\ell^p$ ball of the clean input. After the computation of \eqref{eq:PGD} for each restart, a restart that successfully fools our model is chosen.

A modified version of PGD is called Carlini-Wagner (C\&W) attack. In this attack, the loss function $\mathcal{L}$ is taken as the difference between the logit that corresponds to the correct label and the maximum of logits among the incorrect labels. 

{\bf Blackbox attacks} do not assume full knowledge of the model and weights. Decision-based black box models assume access to the decision outputs of the model \citep{brendel2017decision},
while purely blackbox models assume only access to the training dataset, typically using a surrogate model (transfer blackbox) trained on the same dataset in order to generate attacks \citep{tramer2017space}.

==> arxiv/conclusion.tex <==
%!TEX root = ms.tex

\section{Conclusion}

The promising results obtained with our sparse coding frontend open up an exciting new direction for building bottom-up defenses to make neural networks more robust for a wider range of attacks: we can tune our defense to approach the performance of state-of-the-art adversarial training for $\ell^{\infty}$ bounded attacks, while also providing robustness against $\ell^2$ and $\ell^1$ bounded attacks.  The ideas that our defense is based on could be applied to not only the first layer, but also to intermediate layers within neural networks. Such an approach could distribute the workload of combatting attacks across layers, and potentially make the networks more robust to a variety of attacks from within, without the need for adversarial training adapted to a specific class of attacks.


==> arxiv/evaluation.tex <==
%!TEX root = ms.tex

\section{Evaluation}\label{sec:evaluation}

State-of-the-art PGD attacks are based on gradient computation, and an important criticism of prior proposals of preprocessing-based defense is that they were masking/obfuscating/shattering 
gradients, without adapting the attacks to compensate for this \citep{obfuscated-gradients}. Indeed, many such defenses do fail when attacks are suitably adapted, leading a group of prominent
researchers to propose guidelines for evaluating defenses \citep{onevaluating2019}. Following such guidelines, we devote substantial effort to devising attacks adapted to our defense as follows:
\begin{itemize}
	\item Consider several different smooth backward pass replacements for the parts of our defense that are non-differentiable:
		\begin{itemize}
			\item for the activation function, we test two backward passes: identity and a smooth approximation. 
			\item for top $T$ taking operation, we test identity backward pass as well as propagating gradients through top $U$ coefficients where $U>T$.
		\end{itemize}
	\item Check that there exist some $\epsilon$ values that reduce the adversarial accuracy to 0. (see Fig.~\ref{fig:acc_vs_eps})
	\item Test our defense against attacks with large number of iterations or restarts.
	\item Test against different threat models such as: $\ell^\infty$, $\ell^2$, and $\ell^1$ bounded attacks; decision and query based blackbox attacks that do not rely on gradients; transfer blackbox attacks with many different surrogate models
	\item To ensure that the gradients are computed appropriately, we test computing smoothed gradients where gradients are averaged over many different points in the neighborhood of the original point, in each step of the attack. However, we observe that this does not significantly increase the attack strength.
\end{itemize}


==> arxiv/experiments.tex <==
%!TEX root = ms.tex

\section{Experiments and Results}

\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{3pt}
\begin{table}[!b]\centering
\begin{small}
\begin{tabular}{r@{\hspace{15pt}}ccccccc}
\toprule

& Clean & \makecell{Whitebox \\ ($\ell^\infty$, $\epsilon=\frac{8}{255}$)}& \makecell{Whitebox (C\&W) \\ ($\ell^\infty$, $\epsilon=\frac{8}{255}$)}  & \makecell{Whitebox \\ ($\ell^2$, $\epsilon=0.6$)}   &  \makecell{Whitebox \\ ($\ell^1$, $\epsilon=30$)}  & \makecell{Decision \\ Boundary BB}    \\

\midrule
Natural & \bf{92.66} & \phantom{0}0.00 & \phantom{0}0.00 & \phantom{0}0.00 & \phantom{0}0.00 & $\overline{||\mathbf{e}||_2}=0.11$\\
Adv. Training & 79.41 & 43.27 & 42.03 & 52.09 & 19.98 & $\overline{||\mathbf{e}||_2}=0.88$\\
TRADES & 75.17 & \bf{45.79} & \bf{42.87} & 51.35 & 21.15 & $\overline{||\mathbf{e}||_2}=0.91$\\
$T=15$ (Ours) & 85.45 & 37.33 & 37.35 & \bf{60.47} & \bf{47.13} & $\overline{||\mathbf{e}||_2}=\bf{3.04}$\\


\bottomrule
\end{tabular}
\end{small}
\caption{Performance (accuracies and norms) of different defense methods (CIFAR-10) }
\label{table:different_defenses}
\end{table} 

We test our defense against a wide range of attacks and compare the results with benchmark defenses from the literature using the CIFAR-10 dataset (pixels scaled between 0 and 1). The benchmarks are PGD adversarially trained \citep{madry2017towards} and TRADES \citep{zhang2019theoretically} defenses for the same classifier architecture under $\ell^{\infty}$ bounded attacks. See Appendix~\ref{sec:hyper} for choice of hyperparameters and training settings for both our defense and benchmarks. Note that the classifier CNN used in our paper is "simpler" ResNet-32 rather than the wide ResNet-32, both of which are utilized in \cite{madry2017towards} and other studies in the literature. The choice of the smaller ResNet-32 network makes evaluation of stronger attacks computationally more feasible.

Table~\ref{table:different_defenses} compares our defense with the benchmarks from the literature (all columns except the last report classification accuracies). In all whitebox attacks, we use attack settings: number of steps $N_s=40$, number of random restarts $N_r=100$ and step size $\delta=\epsilon/8$. For the attacks against our defense, we also use $U=2T$ and backward pass smoothing mentioned in Section~\ref{sec:evaluation} to make it stronger. See Appendix~\ref{sec:attack_details} for discussion of these choices and accuracies for other attack variations. Column~1 reports on clean accuracy. In columns 2 and 3, we report results for the $\ell^\infty$ bounded whitebox attack with cross entropy loss and Carlini-Wagner loss, respectively.  
In columns 4 and 5, we report results for $\ell^2$ and $\ell^1$ bounded attacks, respectively. For the last (sixth) column, we use a decision-based blackbox attack \citep{brendel2017decision} and report the average $\ell^2$ norm of perturbations that brings the classification accuracy to $\sim0.01\%$. This attack does not rely on gradient computation. For a given datapoint, the starting point for the perturbation search in this attack is chosen as the closest (in the $\ell^2$ sense) datapoint with a different label. Other parameters for this attack are the default parameters in \texttt{foolbox} \citep{rauber2017foolboxnative} Python package.

We highlight the following observations from Table~\ref{table:different_defenses}: (a) the clean accuracy (column 1) is better than that of the benchmarks, (b) the adversarial accuracy (columns 2 and 3) for $\ell^{\infty}$ bounded perturbations falls short of the benchmarks, (c) the adversarial accuracy for $\ell^2$ (column 4) and $\ell^1$ (column 5) bounded perturbations is substantially better than that of the benchmarks, (d) the average $\ell_2$ norm (column 6) required to create a classification error with high probability with a non-gradient attack is substantially higher for our defense. 

The robustness of our defense to $\ell^{p}$ attacks with different $p$ is because the impact of different attacks is similar: they flip $\pm1$ to $0$ and $0$ to $\pm1$ in the sparse code.
In contrast, standard adversarial training approaches are optimized for $\ell^p$ bounded attacks for a specific $p$, and do not perform as well under other types of attacks.


==> arxiv/frontend.tex <==
%!TEX root = ms.tex

\vspace*{-0.03cm}
\section{Frontend}\label{sec:frontend}

We consider RGB images of size $N \times N \times 3$, processed using  $n \times n \times 3$ patches with stride $S$, so that we process $M = m \times m$ patches, where $m =\lfloor{(N-n)/S}\rfloor +1$. 
We learn a patch-level overcomplete dictionary (number of basis tensors much larger than the patch dimension $3 n^2$) in unsupervised fashion, and use it to extract sparse local features. These outputs go through a CNN ``decoder'' whose goal is to restore the output
dimension to $N \times N \times 3$ rather than to reconstruct the image. This frontend is followed by a standard CNN classifier, trained jointly with the decoder using standard supervised learning. 

\vspace*{-0.03cm}
\subsection{Patch-level Overcomplete Dictionary}

We use a standard algorithm \citep{mairal2009online} (implemented in Python library \texttt{scikit-learn}) which is a variant of K-SVD \citep{elad2006image}. 
Given a set of clean training images $\mathcal{X}=\{\mathbf{X}^{(k)}\}_{k=1}^{K}$, an overcomplete dictionary $\mathbf{D}$ with $L$ atoms is learnt by solving the following optimization problem \citep{mairal2009online}:
\begin{equation}\label{eq:Dict}
\min _{\mathbf{D} \in \mathcal{C}, \{\boldsymbol{\alpha^{(k)}}\}_{k=1}^{K}} \sum_{k=1}^{K}\sum_{i,j}\Bigl( \frac{1}{2}\left\|\mathbf{R}_{ij}\mathbf{X}^{(k)}-\mathbf{D} \boldsymbol{\alpha}_{ij}^{(k)}\right\|_{2}^{2} +\lambda\left\|\boldsymbol{\alpha}_{ij}^{(k)}\right\|_{1}\Bigr)
\end{equation}
where $\mathcal{C} \triangleq \bigl\{\mathbf{D} = [\mathbf{d}_{1}, \ldots, \mathbf{d}_{L}] \in \mathbb{R}^{\bar{n} \times L} \mid \left\|\mathbf{d}_{l}\right\|_{2} = 1\,, \forall l \in \{1, \ldots, L \} \bigr\}$, $\lambda$ is a regularization parameter, $\boldsymbol{\alpha}^{(k)}$ is an $m \times m \times L$ tensor containing the coefficients of the sparse decomposition, and $\mathbf{R}_{ij} \in \mathbb{R}^{\bar{n} \times \bar{N}}$ with $\bar{n} \triangleq 3n^2$ and $\bar{N} \triangleq 3N^2$ extracts the $(ij)$-th patch from image $\mathbf{X}^{(k)}$. The optimization problem in \eqref{eq:Dict} is then solved for the two variables $\mathbf{D}$ and $\{\boldsymbol{\alpha}^{(k)}\}_{k=1}^{K}$ in an alternating fashion \citep{mairal2009online,elad2006image}.

The learnt dictionary atoms form the first layer of our frontend, so that the first layer outputs are the projections of the patches onto the atoms.
Specifically, for a given image $\mathbf{X}$, patch $\mathbf{x}_{ij} \in \mathbb{R}^{\bar{n}}$ is extracted based on the $(ij)$-th block of $\mathbf{X}$; that is, $\mathbf{x}_{ij} = \mathbf{R}_{ij}\mathbf{X}$, and then projected onto dictionary $\mathbf{D}$ in order to obtain projection vector $\mathbf{\tilde{x}}_{ij}$, where $\mathbf{\tilde{x}}_{ij} = \mathbf{D}^T\mathbf{x}_{ij}$. 

Since the dictionary is highly overcomplete, the majority of coefficients are relatively small, and a sparse representation of the patch can be obtained from a subset of the coefficients taking large values.
Fig.~\ref{fig:correlations} contrasts the typical distribution of coefficients from our dictionary to that for the first layer for a typical CNN (the latter is not amenable to sparse coding).


\begin{figure}[b]
\centering
\begin{subfigure}{.545\textwidth}
  \centering
  \includegraphics[width=.97\linewidth]{figures/correlations_normalized.pdf}
  \caption{}
  \label{fig:correlations}
\end{subfigure}%
\begin{subfigure}{.455\textwidth}
  \centering
  \includegraphics[width=.97\linewidth]{figures/acc_vs_eps.pdf}
  \caption{}
  \label{fig:acc_vs_eps}
\end{subfigure}
\caption{(a) Histogram of correlations for a typical patch with atoms of an overcomplete dictionary vs. that of activations through layer 1 filters of a standard classifier CNN. (b) Accuracy vs $\epsilon$ plot for our defense ($T=15$) under $\ell^\infty$ PGD attack with various $\epsilon$ values.}
\label{fig:ensemble_benefit}
\end{figure}

\vspace*{-0.03cm}

\subsection{Coefficient Selection and Activation}\label{sec:topT_activation}

For each patch, we keep only the $T$ elements of the projection vector with largest absolute values, zeroing out the remaining elements, limiting the dimension of the subspace available to the adversary. The surviving coefficients are denoted by $\mathbf{\hat{x}}_{ij}$. Next, in order to ensure that the adversarial perturbations cannot ride on top of the signal in the surviving coefficients $\mathbf{\hat{x}}_{ij}$, we apply an activation function, zeroing out coefficients smaller than a threshold, and keeping only the sign of coefficients passing the threshold. 
The specific design we consider targets $\ell^{\infty}$ bounded perturbations of size $\epsilon$ (but as we shall see, provides robustness against $\ell^2$ and $\ell^1$ bounded perturbations as well):
we set the threshold for atom $\mathbf{d}_{l}$  to be a multiple of $\epsilon \left\|\mathbf{d}_{l}\right\|_{1}$, the maximum possible contribution of 
of such a perturbation to the output. 
\begin{equation}\label{eq:act_fun}
\mathbf{\bar{x}}_{ij}(l)=\biggl\{\begin{array}{ll}
\sign{(\mathbf{\hat{x}}_{ij}(l))}\left\|\mathbf{d}_{l}\right\|_{1}, & \text { if } \frac{|\mathbf{\hat{x}}_{ij}(l)|}{\epsilon \left\|\mathbf{d}_{l}\right\|_{1}} \geq \beta\\
0, & \text{otherwise}
\end{array},
\end{equation}
for all $l \in\{1, \ldots, L\}$, where $\beta > 1$ is a hyperparameter. The scaling of the surviving $\pm 1$ outputs by $\left\|\mathbf{d}_{l}\right\|_{1}$ 
allows basis coefficients surviving a larger $\ell^1$ norm based threshold to contribute more towards the decoder input, but could be omitted, since the decoder can learn the appropriate weights.


\subsection{Decoder}

The discretized sparse codes $\mathbf{\bar{x}}_{ij}$ are fed into a CNN decoder with three transposed convolution layers followed by ReLU activations after each layer, which restores the original image size.

==> arxiv/introduction.tex <==
%!TEX root = ms.tex

\section{Introduction}\label{sec:introduction}

Deep neural networks (DNNs) are known to be vulnerable to small, adversarially designed perturbations \citep{biggio2013evasion, szegedy2013intriguing}.
Since the discovery of such adversarial
attacks, researchers have tried various defense strategies such as adversarial training \citep{madry2017towards,zhang2019theoretically}, constraining Lipschitz constant \citep{cisse2017parseval}, randomized smoothing \citep{cohen2019certified}, and preprocessing methods \citep{guo2017countering,yang2019me}. Sadly, the majority of the proposed defenses have been subsequently defeated \citep{carlini2017adversarial,obfuscated-gradients}.  Current state-of-the-art defenses, as determined by several independent research efforts, are variants of adversarial training \citep{zhang2019theoretically,carmon2019unlabeled}. 

In this paper, we propose, and extensively evaluate on the CIFAR-10 image dataset, a novel preprocessing defense trained only on clean images.
We employ sparse coding using an overcomplete patch-level dictionary, and mitigate adversarial perturbations by (1) zeroing out all but the top $T$ coefficients of the basis projection, thus restricting the attack space, and
(2) quantizing the surviving coefficients to $\pm 1$, thus not allowing perturbations to ride on top of them.  The defense parameters are chosen to combat $\ell^{\infty}$ bounded
attacks, but we demonstrate its general-purpose nature by showing that it also provides robustness against $\ell^2$ and $\ell^1$ bounded attacks. The code for our defense can be found at: \url{https://github.com/canbakiskan/sparse_coding_frontend}


==> arxiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

